Understanding the Social Context of Eating with Multimodal Smartphone Sensing: The Role of Country Diversity

Understanding the social context of eating is crucial for promoting healthy eating behaviors. Multimodal smartphone sensor data could provide valuable insights into eating behavior, particularly in mobile food diaries and mobile health apps. However, research on the social context of eating with smartphone sensor data is limited, despite extensive studies in nutrition and behavioral science. Moreover, the impact of country differences on the social context of eating, as measured by multimodal phone sensor data and self-reports, remains under-explored. To address this research gap, our study focuses on a dataset of approximately 24K self-reports on eating events provided by 678 college students in eight countries to investigate the country diversity that emerges from smartphone sensors during eating events for different social contexts (alone or with others). Our analysis revealed that while some smartphone usage features during eating events were similar across countries, others exhibited unique trends in each country. We further studied how user and country-specific factors impact social context inference by developing machine learning models with population-level (non-personalized) and hybrid (partially personalized) experimental setups. We showed that models based on the hybrid approach achieve AUC scores up to 0.75 with XGBoost models. These findings emphasize the importance of considering country differences in building and deploying machine learning models to minimize biases and improve generalization across different populations.

==> Sections/Tables/features.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
\caption{Summary of 105 features extracted from sensing data, aggregated around activity self-reports using a time window. Detailed information can be found in \cite{generalization_across_countries}. }
\label{table_features}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lll@{}}

\rowcolor[HTML]{EDEDED}
\textbf{Modality} &
  \textbf{Frequency} &
  \textbf{Corresponding features and description} \\ 

Activity &
  \begin{tabular}[c]{@{}l@{}}2 samples \\ per minute\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Derived by Google Activity Recognition API. Measures time \\ spent doing activities: still / in vehicle / on bicycle / on foot / running / tilting / \\ walking / other.\end{tabular} \\

\arrayrulecolor{Gray}
    \midrule
    
App events &
  \begin{tabular}[c]{@{}l@{}}10 samples \\ per minute\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Time spent on apps grouped by categories derived from Google Play Store: \\ action / adventure / arcade /  art \& design / auto \& vehicles /  beauty / board / \\ books \& reference / business / card / casino / casual / comics / communication /  \\ dating /  education / entertainment / finance / food \& drink / health \& fitness / house / \\ lifestyle / maps \& navigation / medical / music / news \& magazine / parenting /\\ personalization / photography / productivity / puzzle / racing / role playing / shopping / \\ simulation / social / sports / strategy / tools / travel / trivia / video players \& editors / \\ weather / word / not found\end{tabular} \\
  \arrayrulecolor{Gray}
    \midrule
    
\begin{tabular}[c]{@{}l@{}}Bluetooth \\ {[}low energy, \\ normal{]}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}1 sample \\ per minute\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Number of devices: total number of Bluetooth devices detected \\ Mean/Std/Min/Max of Received Signal Strength Indication (RSSI) : measures the \\ proximity of other existing devices.\end{tabular} \\
\arrayrulecolor{Gray}
    \midrule
\begin{tabular}[c]{@{}l@{}}Cellular {[}GSM, \\ WCDMA, LTE{]}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}1 sample \\ per minute\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Number of devices : total number of devices detected \\ Mean/Std/Min/Max of Phone signal strength\end{tabular} \\
  \arrayrulecolor{Gray}
    \midrule
Location &
  \begin{tabular}[c]{@{}l@{}}1 sample \\ per minute\end{tabular} &
  Radius of gyration, Distance traveled, Mean/Std/Min/Max Altitude \\
\arrayrulecolor{Gray}
    \midrule
Notifications &
  on change &
  \begin{tabular}[c]{@{}l@{}}Notifications posted: number of incoming notifications \\ Notifications removed: number of notifications removed by the user \\ (features calculated with and without duplicates)\end{tabular} \\
  \arrayrulecolor{Gray}
    \midrule
Proximity &
  \begin{tabular}[c]{@{}l@{}}10 samples \\ per second\end{tabular} &
  Mean/Std/Min/Max of Proximity sensor values \\
\arrayrulecolor{Gray}
    \midrule 
Screen events &
  on change &
  \begin{tabular}[c]{@{}l@{}}Number of screen episodes, Mean/Min/Max/Std of Episode Time (an episode \\ indicates the period from the time the screen turns on until it turns off)\\ Total time: total screen time during the time window\end{tabular} \\
  \arrayrulecolor{Gray}
    \midrule
    
Steps &
  \begin{tabular}[c]{@{}l@{}}10 samples \\ per second \\ or on change\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Step counter : derived using the total number of steps since the last \\ time phone turned on. \\ Steps detected: derived using event-trigger for each new step\end{tabular} \\

\arrayrulecolor{Gray}
    \midrule
Touch events &
  on change &
  Number of touch events \\

  \arrayrulecolor{Gray}
    \midrule
User presence &
  on change &
  \begin{tabular}[c]{@{}l@{}}Derived using android API, indicates the amount of time the phone was used during the \\ time window (referred as user presence).\end{tabular} \\
\arrayrulecolor{Gray}
    \midrule
    
WiFi &
  \begin{tabular}[c]{@{}l@{}}1 sample \\ per minute\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Connected to a network indicator /  Number of devices detected \\ Mean/Std/Min/Max of Received Signal Strength Indication (RSSI)\end{tabular} \\ 
  
  \arrayrulecolor{Gray}
    \bottomrule
\end{tabular}%
}
\end{table}

==> Sections/Tables/models_wo_randbaseline.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\caption{Mean ($\overline{A}$) and Standard Deviation ($A_{\sigma}$) of inference AUCROC for population level models and hybrid models, calculated with XGBoost and Baseline (trained on time based features)}
\label{tab:table-merged}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{lllll}
 &
  \multicolumn{2}{c|}{\cellcolor[HTML]{9FBAC1}\textbf{Population Level}} &
  \multicolumn{2}{c}{\cellcolor[HTML]{B1CBD2}\textbf{Hybrid}} \\
 &
  \cellcolor[HTML]{C0C0C0}{\color[HTML]{343434} Model} &
  \cellcolor[HTML]{C0C0C0}{\color[HTML]{343434} Baseline} &
  \cellcolor[HTML]{C0C0C0}{\color[HTML]{343434} Model} &
  \cellcolor[HTML]{C0C0C0}{\color[HTML]{343434} Baseline} \\ 
\rowcolor[HTML]{FFFFFF} 
China    & .48 (.05) & .47 (.03) & .68 (.02) & .50 (.02)          \\
\rowcolor[HTML]{EFEFEF} 
Denmark  & .52 (.08) & .50 (.06) & .74 (.04) & .57 (.03)          \\
India    & .50 (.04) & .49 (.03) & .75 (.06) & \textit{.58 (.05)} \\
\rowcolor[HTML]{EFEFEF} 
Italy    & .58 (.01) & .57 (.02) & .64 (.01) & .57 (.01)          \\
Mexico   & .53 (.05) & .51 (.06) & .65 (.03) & .57 (.01)          \\
\rowcolor[HTML]{EFEFEF} 
Mongolia & .49 (.01) & .50 (.01) & .57 (.01) & .50 (.01)          \\
Paraguay & .49 (.06) & .55 (.05) & .61 (.04) & .55 (.03)          \\
\rowcolor[HTML]{EFEFEF} 
Uk       & .55 (.04) & .53 (.03) & .75 (.04) & .56 (.02)          \\ \hline
Americas & .53 (.02) & .51 (.04) & .63 (.03) & .54 (.02)          \\
\rowcolor[HTML]{EFEFEF} 
Asia     & .51 (.06) & .52 (.04) & .72 (.03) & .55 (.04)          \\
Europe   & .56 (.05) & .54 (.03) & .72 (.04) & .56 (.02)          \\
\rowcolor[HTML]{EFEFEF} 
Multi-Country    & .53 (.03) & .53 (.02) & .69 (.02) & .53 (.02)         
\end{tabular}%
}
\vspace{-0.2 in}
\end{table}
